EcoAgent: An Efficient Device-Cloud Collaborative Multi-Agent Framework for Mobile Automation

To tackle increasingly complex tasks, recent research on mobile agents has shifted towards multi-agent collaboration. Current mobile multi-agent systems are primarily deployed in the cloud, leading to high latency and operational costs. A straightforward idea is to deploy a device-cloud collaborative multi-agent system, which is nontrivial, as directly extending existing systems introduces new challenges: (1) reliance on cloud-side verification requires uploading mobile screenshots, compromising user privacy; and (2) open-loop cooperation lacking device-to-cloud feedback, underutilizing device resources and increasing latency. To overcome these limitations, we propose EcoAgent, a closed-loop device-cloud collaborative multi-agent framework designed for privacy-aware, efficient, and responsive mobile automation. EcoAgent integrates a novel reasoning approach, Dual-ReACT, into the cloud-based Planning Agent, fully exploiting cloud reasoning to compensate for limited on-device capacity, thereby enabling device-side verification and lightweight feedback. Furthermore, the device-based Observation Agent leverages a Pre-understanding Module to summarize screen content into concise textual descriptions, significantly reducing token usage and device-cloud communication overhead while preserving privacy. Experiments on AndroidWorld demonstrate that EcoAgent matches the task success rates of fully cloud-based agents, while reducing resource consumption and response latency. Our project is available here: https://github.com/Yi-Biao/EcoAgent.

==> src/4f_Case_study.tex <==
\subsection{Case Study}

\begin{figure*}[htbp]
  \centering
  \includegraphics[width=\linewidth]{figures/casestudy}
  \caption{A complete case of EcoAgent executing the ContactsAddContact task in AndroidWorld. The figure illustrates the full interaction loop among Planning, Execution, and Observation Agents across multiple steps until task completion.}
  \label{fig:casestudy}
\end{figure*}

Figure~\ref{fig:casestudy} illustrates the complete operational process of \textbf{EcoAgent} in executing complex multi-step tasks on mobile devices.  The Planning Agent first retrieves the user instruction and the initial screen from the edge, then generates an initial plan using a Dual-ReAct formulation. This plan is transmitted to both the Execution Agent and the Observation Agent.

The Execution Agent and Observation Agent collaborate by alternately performing actions and evaluating outcomes based on step-wise expectations. At each step, the Observation Agent converts the screen into a compact semantic representation via the Pre-Understanding Module. When an unexpected scenario occurs, such as a permission popup not included in the original plan, the Observation Agent identifies the failure and transmits the corresponding textual representation to the cloud-based Memory Module. This information, together with the Reflection Module, assists the Planning Agent in performing replanning. The new plan is adapted to the current mobile environment and guides the two edge-based agents to continue execution accordingly.

As shown in the example, most of the nine-step task is completed on-device. The cloud-based agent is triggered only twice, and aside from the initial planning, communication between edge and cloud remains lightweight and textual, supporting low-bandwidth yet effective collaboration.
